The Automated Inspection of Opaque Liquid Vaccines

In the pharmaceutical industry the screening of opaque vaccines containing suspensions is currently a manual task carried out by trained human visual inspectors. We show that deep learning can be used to effectively automate this process. A moving contrast is required to distinguish anomalies from other particles, reflections and dust resting on a vial's surface. We train 3D-ConvNets to predict the likelihood of 20-frame video samples containing anomalies. Our unaugmented dataset consists of hand-labelled samples, recorded using vials provided by the HAL Allergy Group, a pharmaceutical company. We trained ten randomly initialized 3D-ConvNets to provide a benchmark, observing mean AUROC scores of 0.94 and 0.93 for positive samples (containing anomalies) and negative (anomaly-free) samples, respectively. Using Frame-Completion Generative Adversarial Networks we: (i) introduce an algorithm for computing saliency maps, which we use to verify that the 3D-ConvNets are indeed identifying anomalies; (ii) propose a novel self-training approach using the saliency maps to determine if multiple networks agree on the location of anomalies. Our self-training approach allows us to augment our data set by labelling 217,888 additional samples. 3D-ConvNets trained with our augmented dataset improve on the results we get when we train only on the unaugmented dataset.

==> saliency/19360/19360.tex <==
\begin{table*}
        
        \centering
        \resizebox{\textwidth}{!}{%
        \bgroup
        \footnotesize
        \tabulinesep=0.5mm
        \begin{tabu}{|p{2cm}|c|c|c|c|c|c|c|c|c|c|}
            \hline
            Time-step & 1 & 3 & 5 & 7 & 9 & 11 & 13 & 15 & 17 & 19 \\
            \hline
            
            Saliency:

            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19360/gsStack_SSGANs_masklen_40_0.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19360/gsStack_SSGANs_masklen_40_2.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19360/gsStack_SSGANs_masklen_40_4.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19360/gsStack_SSGANs_masklen_40_6.jpg}}
            &
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19360/gsStack_SSGANs_masklen_40_8.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19360/gsStack_SSGANs_masklen_40_10.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19360/gsStack_SSGANs_masklen_40_12.jpg}}
            &
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19360/gsStack_SSGANs_masklen_40_14.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19360/gsStack_SSGANs_masklen_40_16.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19360/gsStack_SSGANs_masklen_40_18.jpg}}            
            \\
            \hline
        \end{tabu}\egroup}
        \caption{Trajectory of an aggregate}
        \label{tbl:saliency:trajectory}
    \end{table*}

==> saliency/19405/19405.tex <==
\begin{table*}
        
        \centering
        \resizebox{\textwidth}{!}{%
        \bgroup
        \footnotesize
        \tabulinesep=0.5mm
        \begin{tabu}{|p{2cm}|c|c|c|c|c|c|c|c|c|c|}
            \hline
            Time-step & 1 & 3 & 5 & 7 & 9 & 11 & 13 & 15 & 17 & 19 \\
            \hline
            
            Saliency:

            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19405/gsStack_CNN3D_masklen_40_0.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19405/gsStack_CNN3D_masklen_40_2.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19405/gsStack_CNN3D_masklen_40_4.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19405/gsStack_CNN3D_masklen_40_6.jpg}}
            &
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19405/gsStack_CNN3D_masklen_40_8.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19405/gsStack_CNN3D_masklen_40_10.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19405/gsStack_CNN3D_masklen_40_12.jpg}}
            &
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19405/gsStack_CNN3D_masklen_40_14.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19405/gsStack_CNN3D_masklen_40_16.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19405/gsStack_CNN3D_masklen_40_18.jpg}}            
            \\
            \hline
        \end{tabu}\egroup}
        \caption{Example with reflections (top and bottom left corners)}
        \label{tbl:saliency:trajectory}
    \end{table*}

==> saliency/19515/19515.tex <==
\begin{table*}
        
        \centering
        \resizebox{\textwidth}{!}{%
        \bgroup
        \footnotesize
        \tabulinesep=0.5mm
        \begin{tabu}{|p{2cm}|c|c|c|c|c|c|c|c|c|c|}
            \hline
            Time-step & 1 & 3 & 5 & 7 & 9 & 11 & 13 & 15 & 17 & 19 \\
            \hline
            
            Saliency:

            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19515/gsStack_SSGANs_masklen_20_0.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19515/gsStack_SSGANs_masklen_20_2.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19515/gsStack_SSGANs_masklen_20_4.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19515/gsStack_SSGANs_masklen_20_6.jpg}}
            &
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19515/gsStack_SSGANs_masklen_20_8.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19515/gsStack_SSGANs_masklen_20_10.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19515/gsStack_SSGANs_masklen_20_12.jpg}}
            &
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19515/gsStack_SSGANs_masklen_20_14.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19515/gsStack_SSGANs_masklen_20_16.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19515/gsStack_SSGANs_masklen_20_18.jpg}}            
            \\
            \hline
        \end{tabu}\egroup}
        \caption{Small fibre}
        \label{tbl:saliency:trajectory}
    \end{table*}

==> saliency/19755/19755.tex <==
\begin{table*}
        
        \centering
        \resizebox{\textwidth}{!}{%
        \bgroup
        \footnotesize
        \tabulinesep=0.5mm
        \begin{tabu}{|p{2cm}|c|c|c|c|c|c|c|c|c|c|}
            \hline
            Time-step & 1 & 3 & 5 & 7 & 9 & 11 & 13 & 15 & 17 & 19 \\
            \hline
            
            Saliency:

            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19755/gsStack_SSGANs_masklen_20_0.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19755/gsStack_SSGANs_masklen_20_2.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19755/gsStack_SSGANs_masklen_20_4.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19755/gsStack_SSGANs_masklen_20_6.jpg}}
            &
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19755/gsStack_SSGANs_masklen_20_8.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19755/gsStack_SSGANs_masklen_20_10.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19755/gsStack_SSGANs_masklen_20_12.jpg}}
            &
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19755/gsStack_SSGANs_masklen_20_14.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19755/gsStack_SSGANs_masklen_20_16.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{saliency/19755/gsStack_SSGANs_masklen_20_18.jpg}}            
            \\
            \hline
        \end{tabu}\egroup}
        \caption{Small fibre}
        \label{tbl:saliency:trajectory}
    \end{table*}

==> sequences/19094.tex <==
\begin{table*}
        
        \centering
        \resizebox{\textwidth}{!}{%
        \bgroup
        \footnotesize
        \tabulinesep=0.5mm
        \begin{tabu}{|p{2cm}|c|c|c|c|c|c|c|c|c|c|}
            \hline
            Time-step & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
            \hline
            
            Ground Truth

            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/original0.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/original1.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/original2.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/original3.jpg}}
            &
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/original4.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/original5.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/original6.jpg}}
            &
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/original7.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/original8.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/original9.jpg}}            
            \\
            \hline
            
            FC-GANs output after masking bottom right corner

            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/fake0.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/fake1.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/fake2.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/fake3.jpg}}
            &
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/fake4.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/fake5.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/fake6.jpg}}
            &
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/fake7.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/fake8.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/fake9.jpg}}        
            \\
            % \hline
            % Saliency Map
            % & 
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/gsStack_CNN3D_masklen_40_0.jpg}}
            % & 
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/gsStack_CNN3D_masklen_40_1.jpg}}
            % & 
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/gsStack_CNN3D_masklen_40_2.jpg}}
            % & 
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/gsStack_CNN3D_masklen_40_3.jpg}}
            % &
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/gsStack_CNN3D_masklen_40_4.jpg}}
            % & 
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/gsStack_CNN3D_masklen_40_5.jpg}}
            % & 
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/gsStack_CNN3D_masklen_40_6.jpg}}
            % &
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/gsStack_CNN3D_masklen_40_7.jpg}}
            % & 
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/gsStack_CNN3D_masklen_40_8.jpg}}
            % & 
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19094/gsStack_CNN3D_masklen_40_9.jpg}}        
            % \\
            \hline
        \end{tabu}\egroup}
        \caption{}
        \label{tbl:saliency_maps}
    \end{table*}

==> sequences/19908.tex <==
\begin{table*}
        
        \centering
        \resizebox{\textwidth}{!}{%
        \bgroup
        \footnotesize
        \tabulinesep=0.5mm
        \begin{tabu}{|p{2cm}|c|c|c|c|c|c|c|c|c|c|}
            \hline
            Time-step & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
            \hline
            
            Ground Truth

            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/original0.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/original1.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/original2.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/original3.jpg}}
            &
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/original4.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/original5.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/original6.jpg}}
            &
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/original7.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/original8.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/original9.jpg}}            
            \\
            \hline
            
            FC-GANs output after masking bottom right corner

            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/fake0.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/fake1.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/fake2.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/fake3.jpg}}
            &
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/fake4.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/fake5.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/fake6.jpg}}
            &
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/fake7.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/fake8.jpg}}
            & 
            \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/fake9.jpg}}        
            \\
            % \hline
            % Saliency Map
            % & 
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/gsStack_CNN3D_masklen_40_0.jpg}}
            % & 
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/gsStack_CNN3D_masklen_40_1.jpg}}
            % & 
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/gsStack_CNN3D_masklen_40_2.jpg}}
            % & 
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/gsStack_CNN3D_masklen_40_3.jpg}}
            % &
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/gsStack_CNN3D_masklen_40_4.jpg}}
            % & 
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/gsStack_CNN3D_masklen_40_5.jpg}}
            % & 
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/gsStack_CNN3D_masklen_40_6.jpg}}
            % &
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/gsStack_CNN3D_masklen_40_7.jpg}}
            % & 
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/gsStack_CNN3D_masklen_40_8.jpg}}
            % & 
            % \raisebox{-.5\height}{\includegraphics[height=1.8cm]{sequences/19908/gsStack_CNN3D_masklen_40_9.jpg}}        
            % \\
            \hline
        \end{tabu}\egroup}
        \caption{}
        \label{fig:FC-GANs:Completed_Region_vs_gt}
    \end{table*}

==> sequences/FCGANs_Example.tex <==
\begin{figure*}
\centering
    \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake0.jpg}}{$t=1$}
    \end{subfigure} 
    \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake1.jpg}}{$t=2$}
    \end{subfigure} 
        \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake2.jpg}}{$t=3$}
    \end{subfigure} 
    \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake3.jpg}}{$t=4$}
    \end{subfigure} 
    %%%%%%%%%%%%%
        \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake4.jpg}}{$t=5$}
    \end{subfigure} 
    \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake5.jpg}}{$t=6$}
    \end{subfigure} 
        \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake6.jpg}}{$t=7$}
    \end{subfigure} 
    \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake7.jpg}}{$t=8$}
    \end{subfigure} 
    %%%%%%%%%%%%%%%%%
         \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake8.jpg}}{$t=9$}
    \end{subfigure} 
    \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake9.jpg}}{$t=10$}
    \end{subfigure}\\
    \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake10.jpg}}{$t=11$}
    \end{subfigure} 
    \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake11.jpg}}{$t=12$}
    \end{subfigure} 
    %%%%%%%%%%%%%%%%% 
    \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake12.jpg}}{$t=13$}
    \end{subfigure} 
    \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake13.jpg}}{$t=14$}
    \end{subfigure} 
        \begin{subfigure}[b]{0.08\textwidth}
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake14.jpg}}{$t=15$}
    \end{subfigure} 
    \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake15.jpg}}{$t=16$}
    \end{subfigure} 
    \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake16.jpg}}{$t=17$}
    \end{subfigure}     
        \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake17.jpg}}{$t=18$}
    \end{subfigure}
        \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake18.jpg}}{$t=19$}
    \end{subfigure}
        \begin{subfigure}[b]{0.08\textwidth}
        \centering
        \stackunder{\includegraphics[width=\textwidth]{sequences/FCGANs_Example/fake19.jpg}}{$t=20$}
    \end{subfigure} 
    %%%%%%%%%%%%%%%%% 
\caption{Example of a frame sequence with a completed region.}
\label{fig:FC-GANs:Completed_Region_Lot_Of_Movement}
\end{figure*} 

